D-LGP: Dynamic Logic-Geometric Program for Reactive Task and Motion Planning

Many real-world sequential manipulation tasks involve a combination of discrete symbolic search and continuous motion planning, collectively known as combined task and motion planning (TAMP). However, prevailing methods often struggle with the computational burden and intricate combinatorial challenges, limiting their applications for online replanning in the real world. To address this, we propose Dynamic Logic-Geometric Program (D-LGP), a novel approach integrating Dynamic Tree Search and global optimization for efficient hybrid planning. Through empirical evaluation on three benchmarks, we demonstrate the efficacy of our approach, showcasing superior performance in comparison to state-of-the-art techniques. We validate our approach through simulation and demonstrate its reactive capability to cope with online uncertainty and external disturbances in the real world. Project webpage: https://sites.google.com/view/dyn-lgp.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

A Logic-Geometric Program (LGP) \cite{toussaint2015logic} is a hybrid optimization problem over both discrete logical variables and continuous geometric variables. Let $x: [0, T] \rightarrow \mathcal{X}$ denotes a path in the configuration space $\mathcal{X} = \mathbb{R} ^n \times SE(3)^n$ of the whole environment, including an $n$-dimensional robot and $m$ manipulated objects. The logical variables are described as $a_{1:K}, s_{1, K}$, corresponding to discrete actions and symbolic states. The continuous variables are denoted as $x(t): t \in \mathbb{R} \rightarrow \mathcal{X}$, corresponding to the system trajectory in continuous domain. The whole path is divided into $K$ phases of a fixed duration $T$, with $s_k$ representing the logical states at phase $k$. A successor function is used for logical state transition, namely $s_k = succ(a_k, s_{k-1})$. The LGP problem is formulated as following:
\begin{equation}
	\begin{small}
	\label{eq:LGP}
	\begin{aligned}
		\min_{a_{1:k}, x(t), u(t)} \quad & \int_0^{KT} c(x(t), u(t)) \, dt + c_T (x(KT), g)\\
		\textrm{s.t.} \quad & x(0) = x_0, s_{K} \in \mathcal{G} (g) \\
		&h_{\text{goal}}(x(KT), g) = 0
		\\
		\forall t \in [0, KT]: \quad &h_{\text{path}}(x(t), u(t) | s_k(t)) = 0 \\ & g_{\text{path}}(x(t), u(t) | s_k(t)) \leq 0 \\
		 \forall k \in 1, \dots,  K: \quad &h_{\text{switch}}(x(t_k) | a_k, s_{k-1}) = 0     \\ & g_{\text{switch}}(x(t_k) \, | \, a_k, s_{k-1}) \leq 0 \\
		 & a_k \in \mathcal{A} (s_{k-1})\\
		 & s_k \in succ(s_{k-1}, a_k),	 
	\end{aligned}
\end{small}
\end{equation}
where $h_{\text{path}}$ and $g_{\text{path}}$ represent the path constraints under each phase, and $h_{\text{switch}}$, $g_{\text{switch}}$ denote the transition conditions between two phases with the action operator $a_k$. $s_{K} \in \mathcal{G}$ and $h_{\text{goal}}$ describes the goal specification logically and geometrically. $c(.)$ and $c_T(.)$ are the path cost and terminal cost to penalize control effort (e.g., energy, force) and the final kinematic performance.

The solution of an LGP is a sequence of symbolic actions $a_{1:k}$ and the corresponding continuous motion variables $u(t)$ and the resulted path trajectory $x(t)$.
\cite{toussaint2015logic} proposed to solve LGPs by breaking the problem into three levels. Tree search is first used in STRIPS domain to find a candidate action skeleton $a_{1:k}$. Next, this action skeleton defines anonlinear program (NLP) with the constraints corresponding to the action skeletons and symbolic states. Solving the continuous full path problem is usually too expensive and the candidate NLPs is usually very high. To address this issue, \cite{toussaint2017multi} proposed to use multi-level different coarse time-discretization strategies for feasibility checking and cost computation to achieve fast monte-carlo tree search, such as pose bound and sequence bound. Pose bound assumes perfect previous path and aims to quickly check the feasibility of current action skeleton. Sequence bound aims to jointly optimize the variables at keyframe step $t_k$, $\forall$ $k=1, \dots, K$, but without considering the full path.





%Next, this action skeleton defines a trajectory optimization problem with the constraints corresponding to the action skeletons and symbolic states:
%\begin{equation}
%\label{eq:NLP}
%	\begin{aligned}
%		\min_{x(t), u(t)} \quad & \int_0^{KT} c(x(t), u(t)) \, dt + c_T (x(KT), g)\\
%		\textrm{s.t.} \quad & x(0) = x_0, h_{\text{goal}}(x(KT), g) = 0
%		\\
%		\forall t \in [0, KT]: \quad &h_{\text{path}}(x(t), u(t) | s_k(t)) = 0 \\ & g_{\text{path}}(x(t), u(t) | s_k(t)) \leq 0.	 
%	\end{aligned}
%\end{equation}
%
%The optimization of the trajectory is a nonlinear program (NLP). Solving the continuous full path problem is usually too expensive and the candidate NLPs is usually very high. To address this issue, \cite{toussaint2017multi} proposed to use multi-level different coarse time-discretization strategies for feasibility checking and cost computation to achieve fast monte-carlo tree search, such as pose bound and sequence bound. Pose bound assumes perfect previous path and aims to quickly check the feasibility of current action skeleton. Sequence bound aims to jointly optimize the variables at keyframe step $t_k$, $\forall$ $k=1, \dots, K$, but without considering the full path.




==> sections/discussion.tex <==
\section{Discussions}
\label{sec:discussion}


